Tensor Decompositions Meet Control Theory: Learning General Mixtures of Linear Dynamical Systems

Recently Chen and Poor initiated the study of learning mixtures of linear dynamical systems. While linear dynamical systems already have wide-ranging applications in modeling time-series data, using mixture models can lead to a better fit or even a richer understanding of underlying subpopulations represented in the data. In this work we give a new approach to learning mixtures of linear dynamical systems that is based on tensor decompositions. As a result, our algorithm succeeds without strong separation conditions on the components, and can be used to compete with the Bayes optimal clustering of the trajectories. Moreover our algorithm works in the challenging partially-observed setting. Our starting point is the simple but powerful observation that the classic Ho-Kalman algorithm is a close relative of modern tensor decomposition methods for learning latent variable models. This gives us a playbook for how to extend it to work with more complicated generative models.

==> mysymbols_backup.tex <==
\newcommand{\tiln}{\widetilde{n}}
\newcommand{\tilp}{\widetilde{p}}
\newcommand{\widetildelta}{\widetilde{\delta}}
\newcommand{\tildelta}{\widetilde{\delta}}
\newcommand{\link}{\Phi}


\newcommand\matnorm[2]{\left|\!\left|\!\left| #1 \right|\!\right|\!\right|_{#2}}
\newcommand\norm[2]{\left|\!\left|#1 \right|\!\right|_{#2}}
\newcommand\trace[1]{\text{tr}\left(#1\right)}
\def\real{\mathbb{R}}
\def\Exp{\mathbb{E}}


% theorem type environments
\newtheorem{theorem}{Theorem}
\newtheorem{condition}{Condition}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{claim}{Claim}


%SpaceSaving Lists
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
       { \setlength{\itemsep}{0pt}      \setlength{\parsep}{1pt}
       \setlength{\topsep}{1pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
       \setlength{\labelsep}{0.5em} } }

\newcommand{\squishenum}[1]{
   \begin{enumerate}[label=(#1\arabic*)]
       { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
       \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
       \setlength{\labelsep}{0.5em} } }



% general symbols
\newcommand{\RF}{\mathbb{R}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\nn}{\nonumber} 
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\sqprn}[1]{\left[ #1 \right]}
\newcommand{\tlprn}[1]{\left\{ #1 \right\}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\tr}[2]{\left<\left< #1 , #2 \right>\right>}
\newcommand{\trs}[2]{\left< #1 , #2 \right>}
\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}
\newcommand{\inprod}[2]{\left\langle #1 , #2 \right\rangle}

\newcommand{\del}{\partial}
\newcommand{\dd}[2]{\frac{d#1}{d#2}}
\newcommand{\ddel}[2]{\frac{\del#1}{\del#2}}
\newcommand{\ddell}[2]{\frac{\del^2#1}{{\del#2}^2}}
\newcommand{\ddelll}[3]{\frac{\del^2#1}{{\del#2}{\del#3}}}
\newcommand{\beq}{\begin{eqnarray*}}
\newcommand{\eeq}{\end{eqnarray*}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\poly}{\text{poly}}

\def \bal#1\eal{\begin{align}#1\end{align}}
\def \bals#1\eals{\begin{align*}#1\end{align*}}

\newcommand{\hide}[1]{}
\newcommand{\oo}[1]{\frac{1}{#1}}
\newcommand{\eps}{\epsilon}
\newcommand{\evalat}[2]{\left.#1\right|_{#2}}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil#1\right\rceil}}
\newcommand{\floor}[1]{\ensuremath{\left\lfloor#1\right\rfloor}}
\newcommand{\ontop}[2]{\overset{{\scriptsize #1}}{#2}}
\newcommand{\Perp}{\perp\!\!\!\perp}
\newcommand{\limsu}{\mathop{\overline{\mathrm{lim}}}}
\newcommand{\limin}{\mathop{\underline{\mathrm{lim}}}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\map}{\mathop{\mathrm{map}}}
\newcommand{\powrs}[1]{\langle\!\langle #1 \rangle\!\rangle}
\newcommand{\polys}[1]{\langle #1 \rangle}
\newcommand{\contf}{\mathscr{C}}
%\newcommand{\trn}{^{{}^\intercal}} %operator transpose
\newcommand{\trn}{^\intercal} %operator transpose
%\newcommand{\trn}{^{{}^{\!\intercal}}} %operator transpose
\newcommand{\inv}{^{-1}} %inverse
\newcommand{\unit}{\boldsymbol{1}}
\newcommand{\zero}{\boldsymbol{0}}
\newcommand{\defeq}{\stackrel{\mathrm{def}}{=}}
\newcommand{\textonTop}[2]{\stackrel{\mathrm{#1}}{#2}}

\newcommand{\pleq}{~+\!=}
\newcommand{\chr}{\mathrm{\bs{1}\hspace{-3pt}I}} % characteristic function
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}

% function names
\newcommand{\zeros}{\mathrm{zeros}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\TR}{\mathrm{tr}}
\newcommand{\vol}{\mathrm{vol}}
\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\acos}{\mathrm{acos}}
\newcommand{\intr}{\mathrm{int}\,}
\newcommand{\extr}{\mathrm{ext}\,}
\newcommand{\dom}{\mathrm{dom}\,}
\newcommand{\conv}{\mathrm{conv}\hspace{1pt}}
\newcommand{\cone}{\mathrm{cone}\hspace{1pt}}


%probability & statistics symbols
\newcommand{\convd}{\overset{{\scriptsize d}}{\to}}
\newcommand{\convp}{\overset{{\scriptsize p}}{\to}}
\newcommand{\unif}{\mathrm{Uniform}}
\newcommand{\bern}{\mathrm{Bernoulli}}
\newcommand{\negbin}{\mathrm{NegBinom}}
\newcommand{\Binom}{\mathrm{Bin}}
\newcommand{\pois}{\mathrm{Poisson}}
%\newcommand{\ndistr}{\mathrm{Normal}}
\newcommand{\ndistr}{\mathrm{n}}
\newcommand{\Bdistr}{\mathrm{Beta}}
\newcommand{\Gdistr}{\mathrm{Gamma}}
% f(x) = \frac{1}{\beta^\alpha\Gamma(\alpha)}x^{\alpha-1}e^{-x/\beta}
\newcommand{\iGdistr}{\mathrm{InvGamma}} 
% f(x) = \frac{1}{\beta^\alpha\Gamma(\alpha)}x^{-\alpha-1}e^{-1/(\beta x)}
\newcommand{\MSE}{\mathrm{MSE}} 
\newcommand{\MAE}{\mathrm{MAE}} 
\newcommand{\ARE}{\mathrm{ARE}} 
\newcommand{\se}{\mathrm{se}} 

%\newcommand{\eg}{\mathrm{e.g.}} 
%\newcommand{\st}{\mathrm{s.t.}} 
%\newcommand{\ie}{\mathrm{i.e.}} 

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\tha}{\theta}
%\newcommand{\mexp}{\mathbb{E}}
%\newcommand{\mexp}[1]{\ensuremath{\text{{\bf E}$\left[#1\right]$}}}
\newcommand{\mexp}{\text{{\bf E}}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\corr}{\mathrm{Cor}}
\newcommand{\bW}{\bs{W}}
\newcommand{\bw}{\bs{w}}
\newcommand{\bX}{\bs{X}}
\newcommand{\bx}{\bs{x}}
\newcommand{\bY}{\bs{Y}}
\newcommand{\by}{\bs{y}}
\newcommand{\bZ}{\bs{Z}}
\newcommand{\bz}{\bs{z}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\ev}{\mathrm{Ev}} %evidence
\newcommand{\pr}{\boldsymbol{\mathrm{P}}}
%\newcommand{\prob}{\mathrm{Pr}}


% embeddings
\newcommand{\embeds}[1]{\;\lhook\joinrel\xrightarrow{#1}\;}

%misc commands
\newcommand{\ds}{\displaystyle}
%\newcommand{\ts}{\textstyle}
\newcommand{\bs}{\boldsymbol}
\renewcommand{\th}{\ensuremath{^{\mathrm{th}}}~}

\usepackage{eso-pic}
\usepackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\st{s.t\onedot} \def\St{\emph{S.t}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\iid{i.i.d}
\def\etal{\emph{et al}\onedot}
\makeatother

% Miscellaneous
\def\naive{na\"\i ve\xspace}
\def\naively{na\"\i vely\xspace}
\def\Naive{Na\"\i ve\xspace}
\def\Naively{Na\"\i vely\xspace}

\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\eqnref}[1]{(\ref{#1})}
\newcommand{\secref}[1]{Section \ref{#1}}
\newcommand{\chapref}[1]{Chapter \ref{#1}}
\newcommand{\thmref}[1]{Theorem \ref{#1}}


%\include{mathmacro}
\makeatletter
\newcommand{\bfgreek}[1]{\bm{\@nameuse{#1}}}
\makeatother

\newcommand{\ind}[1]{[\hspace{-1pt}[#1]\hspace{-1pt}] }
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}

\newenvironment{indentpar}[1]%
     {\begin{list}{}%
             {\setlength{\leftmargin}{#1}}%
             \item[]%
     }
{\end{list}}

\makeatletter
\newcounter{problem}
\newenvironment{problem}[1][]{\refstepcounter{problem}\par\noindent%
\textbf{Problem~\theproblem: #1}}
%\textbf{Problem~\theproblem: #1}\rmfamily}
\makeatother



==> new-algorithm.tex <==
\section{Algorithm}
\label{sec:algorithm}


\begin{mdframed}
  \begin{algorithm}[Learning a Mixture of Linear Dynamical Systems]
    \label{algo:learning-mixture}\mbox{}
    \begin{description}
     \item[Input:] $N$ sample trajectories of length $l$ from a mixture of LDS $\calM = \sum_{i \in [k]} w_i \calL\Paren{A_i, B_i, C_i, D_i}$ denoted $\Set{(y_1^i, \dots , y_l^i)}_{i \in [N]}$, the corresponding control inputs $\Set{(u_1^i, \dots , u_l^i) }_{i \in [N]}$,  parameter $s \in \N$ for individual observability and controllability and joint nondegeneracy, Accuracy parameter $0< \eps<1$ and allowable failure probability $0<\delta<1$. 
     \item[Operation:]\mbox{}
    \begin{enumerate}
    \item Run Algorithm \ref{algo:learning-subspaces} on the input samples  and let $\Set{\wt{G}_i }_{i \in [k]}$ be the matrices returned  
    \textcolor{red}{Allen: Need one additional step to deal with unknown scaling in front.  Here roughly whats happening is $\wt{G}_i = G_iw_i^{1/3}$ and $\wt{w}_i = w_i^{2/3}$}
    \item For $0 \leq k_1 \leq 2s$, compute estimate $\wh{R}_{k_1}$ of $\EE_{\calM}\left[ y_{k_1 + 1} \otimes u_1\right]$ as
    \[
    \wh{R}_{k_1} = \frac{1}{N} \sum_{i = 1}^N y^i_{k_1 + 1} \otimes u_1^i \,.
    \]
    \item Construct estimate $\wh{R}_{\calM}$ of $R_{\calM}$ by stacking together estimates $\wh{R}_{0}, \wh{R}_{1}, \dots , \wh{R}_{2s - 1}$ 
    \item Solve for weights $\wt{w_1}, \dots , \wt{w_k}$ that minimize
    \[
    \norm{\wt{w_1}\wt{G}_1 + \dots + \wt{w_k}\wt{G}_k - R_{\calM} }_F 
    \]
    \item Set $\wh{G}_i = \wt{G}_i/\sqrt{\wt{w_i}}$
    \item Set $\wh{w}_i = \wt{w_i}^{3/2}$ for all $i \in [k]$
    \item Run Algorithm \ref{algo:ho-kalman} on  $\hat{G}_i$ for each $i \in [k]$ to recover parameters $\Set{ \hat{A}_i, \hat{B}_i, \hat{C}_i, \hat{D}_i }_{i \in [k]}$  
    \end{enumerate}
    \item[Output:]  The set of parameter estimates $\Set{\hat{w}_i, \hat{A}_i, \hat{B}_i, \hat{C}_i, \hat{D}_i }_{i \in [k]}$ 
    \end{description}
  \end{algorithm}
\end{mdframed}

In this section, we describe our algorithm for learning a mixture of Linear Dynamical Systems. At a high level, our algorithm uses multiple trajectories to obtain an estimate of the tensor 
\begin{equation*}
\Pi_{\calM} = \sum_{i \in [k]}  w_i G_{\calL_i, 2s} \otimes G_{\calL_i, 2s} \otimes G_{\calL_i, 2s} \,.
\end{equation*}
where 
\begin{equation*}
G_{\calL_i, s} = \begin{bmatrix}
    D_i &  C_i B_i &  C_i A_i B_i &  \ldots & C_i A_i^{s-1}B_i.
    \end{bmatrix}
\end{equation*}

Recall that $G_{\calL_i, 2s}$ has blocks that are of the form $X_{\calL_i, s'}$ for $s' \leq 2s$ and thus it follows from Corollary~\ref{coro:mixture-fourthmoment} that we can construct a unbiased estimates of the individual blocks
\[
T_{s_1, s_2,s_3} = \sum_{i \in [k]}  w_i X_{\calL_i, s} \otimes X_{\calL_i, s_2} \otimes X_{\calL_i, k_1}
\]
of this tensor from the observations and control input.  Piecing together the individual blocks lets us construct an estimate of  $\Pi_{\calM}$. Since we have access to multiple \textit{independent} trajectories, we can show that the variance is bounded and we indeed have access to a tensor close to $\Pi_{\calM}$. 

We then run the classical Jennrich's tensor decomposition algorithm on the tensor $\Pi_{\calM}$ to recover the factors $G_{\calL_i, 2s}$. The key is that the joint nondegeneracy assumption implies that vectors obtained by flattening $G_{\calL_1, 2s}, \dots , G_{\calL_k, 2s }$ are  (robustly) linear independent. Therefore, Jennrich's algorithm indeed recovers the factors $G_{\calL_1, 2s}, \dots , G_{\calL_k, 2s }$.  These are exactly the Markov parameters of the individual components and we can then invoke a robust variant of Ho-Kalman~\cite{oymak2019non} to recover the corresponding parameters.  

Due to some minor technical complications from the unknown mixing weights, it will also be useful to define
\[
R_{\calM} = \sum_{i \in [k]} w_i G_{\calL_i, 2s}
\]
which we can also estimate empirically by estimating each block
\[
R_{s_1} = \EE_{\calM}[y_{k_1 + 1} \otimes u_1] = \sum_{i \in [k]} w_i X_{\calL_i, s_1}
\]
separately.  



\begin{mdframed}
  \begin{algorithm}[Learn Individual Markov Parameters]
    \label{algo:learning-subspaces}\mbox{}
    \begin{description}
     \item[Input:] $N$ sample trajectories of length $l$ from a mixture of LDS $\calM = \sum_{i \in [k]} w_i \calL\Paren{A_i, B_i, C_i, D_i}$, denoted by $\Set{ (y_1^{i}, \ldots y^{i}_{\ell})}_{i \in [N]}$, the corresponding control inputs, denoted $\Set{ (u^{i}_1, \ldots, u^{i}_{\ell})}_{i \in [N]}$,  parameter $s \in \N$ for individual observability and controllability and joint nondegeneracy, accuracy parameter $\eps$ and allowable failure probability $\delta$.
    \item[Operation:]\mbox{}
    \begin{enumerate}
    \item For $0 \leq k_1\leq 2s,0 \leq  k_2 \leq 2s , 0 \leq k_3 \leq 2s$,  
    \begin{enumerate}
    \item Compute empirical estimate $\wh{T}_{k_1,k_2,k_3}$ of
    \[
    \EE_{\calM} [ y_{ k_3 + k_2 + k_1 + 3 } \otimes u_{ k_1 + k_2 + 3} \otimes   y_{k_1 + k_2 + 2} \otimes u_{k_1 + 2} \otimes  y_{k_1 + 1} \otimes u_{1}]
    \] 
    as follows:
    \[
        \wh{T}_{k_1, k_2, k_3} = \frac{1}{N} \sum_{ i \in [n] } y^{i}_{k_1 +k_2 + k_3 + 3 } \otimes u^{i}_{k_1 +k_2 + 3} \otimes y^{i}_{k_1 +k_2 + 2 }\otimes u^{i}_{k_1 + 2} \otimes y^{i}_{k_1 + 1} \otimes u^{i}_1
    \]

    \end{enumerate}
    
    
    \item Construct estimate $\wh{\Pi}_{\calM}$ for $\Pi_{\calM}$ by piecing together the blocks $\wh{T}_{k_1,k_2,k_3}$ appropriately
    \item Flatten pairs of dimensions of $\wh{\Pi}_{\calM}$ so that it is a order-$3$ tensor with dimensions $(2s + 1)mp \times (2s + 1)mp \times (2s+1)mp$ 
    \item Run Jennrich's algorithm (Algorithm \ref{algo:jennrich}) to obtain the following decomposition
    \[
    \wh{\Pi}_{\calM} = \wh{T}_1 + \dots + \wh{T}_k
    \]
    \item For each $\wh{T}_i$, compute the Frobenius norm of each slice in its second and third dimensions to obtain a vector $\wh{v}_i \in \R^{(2s + 1)mp}$ \ainesh{uhhh..how does computing the frobenius norm of the 2nd and 3rd mode help in obtaining $\wh{v}_i$??}
    \item Construct $\wt{G}_i$ by rearranging the vector $\wh{v}_i/\norm{\wh{v}_i}^{2/3}$ back into an $m \times (2s+1)p$ matrix (undoing the flattening operation) \ainesh{if you don't do this reweighting by $\norm{v_i}^{2/3}$ do you lose the weight information? can't you post process to recover the weights?}
    \end{enumerate}
    \item[Output:] Matrices $\wt{G}_1, \dots , \wt{G}_k$
    \end{description}
  \end{algorithm}
\end{mdframed}







\begin{mdframed}
  \begin{algorithm}[Parameter Recovery via Ho-Kalman~\cite{oymak2019non}]
    \label{algo:ho-kalman}\mbox{}
    \begin{description}
    \item[Input:] Parameter $s$, Markov parameter matrix estimate $\hat{G} = [\hat{X}_0, \dots , \hat{X}_{2s}] $  
    
    \item[Operation:]
    %\mbox{State-space realization $\hat{A}, \hat{B}, \hat{C}$}
    \begin{enumerate}
    \item Set $\hat{D} = \hat{X}_0$
    \item Form the Hankel matrix $\hat{H} \in \R^{ms \times p(s+1)}$ from $\hat{G}$ as
    \[
    \hat{H} = \begin{bmatrix} \hat{X}_1 & \hat{X}_2 & \dots & \hat{X}_{s+1} \\ \hat{X}_2 & \hat{X}_3 & \dots & \hat{X}_{s + 2} \\ \vdots & \vdots & \ddots & \vdots \\ \hat{X}_{s} & \hat{X}_{s+1} & \dots & \hat{X}_{2s} 
    \end{bmatrix}
    \]
    \item $\hat{H}^{-} \in \R^{ms \times ps} \leftarrow $ first $ps$ columns of $\hat{H}$
    \item $\hat{L} \in \R^{ms \times ps} \leftarrow$ rank $n$ approximation of $\hat{H}^{-}$ obtained via SVD
    \item $U,\Sigma,V = SVD(\hat{L})$
    \item $\hat{O} \in \R^{ms \times n} \leftarrow U\Sigma^{1/2}$
    \item $\hat{Q} \in \R^{n \times ps} \leftarrow \Sigma^{1/2}V^*$
    \item $\hat{C} \leftarrow$ first $m$ rows of $\hat{O}$
    \item $\hat{B} \leftarrow $ first $p$ column of $\hat{Q}$
    \item $\hat{H}^{+} \in \R^{ms \times ps} \leftarrow $ last $ps$ column of $\hat{H}$
    \item $\hat{A} \leftarrow \hat{O}^{\top} \hat{H}^{+} \hat{Q}^{\top}$
    \end{enumerate}
    \item[Output:] $\hat{A} \in \R^{n \times n}, \hat{B} \in \R^{n \times p}, \hat{C} \in \R^{m \times n}, \hat{D} \in \R^{m \times p}$  
    \end{description}
  \end{algorithm}
\end{mdframed}



\begin{mdframed}
\begin{algorithm}[Jennrich's Algorithm]
\label{algo:jennrich}\mbox{}
\begin{description}
\item[Input:] Tensor $T' \in \R^{n \times n \times n}$ where 
\[
T' = T + E
\]
for some rank-$r$ tensor $T$ and error $E$ \\
\item[Operation:]\mbox{}
\begin{enumerate}
\item Choose unit vectors $a,b \in \R^n$ uniformly at random
\item Let $T^{(a)}, T^{(b)}$ be $n \times n$ matrices defined as 
\begin{align*}
T^{(a)}_{ij} = T'_{i,j , \cdot } \cdot a \\
T^{(b)}_{ij} = T'_{i,j , \cdot } \cdot b
\end{align*}
\item Let $T_r^{(a)}, T_r^{(b)}$ be obtained by taking the top $r$ principal components of $T^{(a)}, T^{(b)}$ respectively.
\item Compute the eigendecompositions of $U = T_r^{(a)}(T_r^{(b)})^+$ and $V = \left((T_r^{(a)})^+T_r^{(b)}\right)^T$ (where for a matrix $M$, $M^+$ denotes the pseudoinverse)
\item Let $u_1, \dots , u_r, v_1, \dots , v_r$ be the eigenvectors computed in the previous step.  
\item Permute the $v_i$ so that for each pair $(u_i,v_i)$, the corresponding eigenvalues are (approximately) reciprocals.
\item Solve the following for the vectors $w_i$
\[
\arg\min \norm{T' - \sum_{i=1}^r u_i \otimes v_i \otimes w_i}_2^2
\]
\end{enumerate}
\item[Output:] the rank-$1$ components $\{u_i \otimes v_i \otimes w_i\}_{i=1}^r$
\end{description}
\end{algorithm}
\end{mdframed}



\section{Analysis}

In this section, we provide the analysis of the algorithms we presented in Section~\ref{sec:algorithm}. 
The main theorem we obtain is as follows:

\begin{theorem}[Learning a Mixture of LDS's]\label{thm:main}
\label{thm:main-thm}
Given $0 < \epsilon, \delta < 1$, an integer $s$, and 
\[
N = \poly\Paren{m,n,p , s, \kappa, 1/w_{\min} ,  1/\gamma, 1/\eps, 1/\delta}
\]
observations $\Set{ (y_1^{i}, \ldots, y_{\ell}^{i} ) }_{i \in [N]}$, and the corresponding control inputs $\Set{ (u_1^{i}, \ldots, u_{\ell}^{i} ) }_{i \in [N]}$ of trajectory length $\ell \geq 6(s+1)$ \ainesh{fix maybe?}, from a mixture of linear dynamical system $\calM = \sum_{i \in [k]} w_i \calL\Paren{ A_i,B_i,C_i,D_i}$, satisfying the assumptions in Section~\ref{sec:formal-setup}, Algorithm \ref{algo:learning-mixture} outputs estimates $\Set{ \hat{A}_i, \hat{B}_i, \hat{C}_i , \hat{D}_i }_{i \in [k]}$ such that with probability at least $1-\delta$, there is a permutation $\pi$ on $[k]$ such that for each $i \in [k]$, there exists a similarity transform $U_i$ satisfying 
\begin{equation*}
\max\Paren{ \Norm{A_{\pi(i)} - U^{-1}_i \hat{A}_i  U_i } , \Norm{C_{\pi(i)} - \hat{C}_iU_i } , \Norm{B_{\pi(i)} - U^{-1}_i \hat{B}_i } , \Norm{D_{\pi(i)} - \hat{D}_i},  \abs{ w_{\pi(i)} - \hat{w}_i }  } \leq \eps. 
\end{equation*}
Further, Algorithm \ref{algo:learning-mixture} runs in $\poly\Paren{m,n,p , s, \kappa, 1/w_{\min} ,  1/\gamma, 1/\eps, 1/\delta}$ time.
    \ainesh{placeholder theorem, fix parameters.}
\end{theorem}


We proceed by analyzing each sub-routine separately. In particular, Algorithm~\ref{algo:learning-mixture} proceeds by first taking the input samples and running Algorithm~\ref{algo:learning-subspaces} to learn the individual sets of Markov parameters up to some scaling by the mixing weights. Formally, 

\begin{theorem}[Recovering the Markov Parameters]
\label{thm:span-recovery}
Given $\eps, \delta>0$ and  
\[N \geq \poly(m, n, p, s, \kappa, 1/w_{\min}, 1/\gamma, 1/\eps,  1/\delta )
\]
trajectories from a mixture of LDS's, $\calM = \sum_{i \in[k]} w_i \calL\Paren{A_i, B_i, C_i, D_i}$,  Algorithm~\ref{algo:learning-subspaces} outputs a set of matrices $\wt{G}_1, \wt{G}_2, \ldots \wt{G}_k$ such that with probability $1 - \delta$, there is a permutation $\pi$ on $[k]$ such that 
\[
\norm{\wt{G}_{\pi(i)} - w_i^{1/3}G_{\calL_i, 2s}}_F \leq \eps 
\]
for all $i \in [k]$.  Further, Algorithm~\ref{algo:learning-subspaces} runs in $\poly(N)$ time.
\end{theorem}

Next, we argue about the mixing weights $\wt{w}_1, \dots , \wt{w}_k$ computed in the regression step in Algorithm~\ref{algo:learning-mixture}.


\begin{theorem}[Recovering the Mixing Weights]
\label{thm:block-henkel-recovery}
Assume that the matrices $\wt{G}_i$ computed in Algorithm~\ref{algo:learning-mixture} satisfy Theorem~\ref{thm:span-recovery}.  Then, with $1 - \delta$ probability, the mixing weights $\wt{w}_1, \dots , \wt{w}_k$ computed in Algorithm~\ref{algo:learning-mixture} satisfy 
\[
|\wt{w}_{\pi(i)} - w_i^{2/3}| \leq \eps \cdot \poly(\kappa,m,n,s,p, 1/\gamma , 1/w_{\min})
\]
for all $i \in [k]$.
\end{theorem}
As a corollary to the above two theorems, the estimates $\wh{G}_i$ computed in Algorithm~\ref{algo:learning-mixture} are actually good estimates for the true individual Markov parameters $G_{\calL_i, 2s}$.  Now, running a stable variant of Ho-Kalman~\cite{oymak2019non} on the individual block Henkel matrices suffices to obtain estimates $\wh{A}_i, \wh{B}_i $, $\wh{C}_i, \wh{D}_i$. Formally, 


\begin{theorem}[Stable Ho-Kalman,~\cite{oymak2019non}]
\label{thm:stable-ho-kalman}
For observability and controllability matrices that are rank $n$, the Ho-Kalman algorithm applied to $\hat{G}$ produces estimates $\hat{A},\hat{B}$, and $\hat{C}$ such that 
there exists similarity transform $T \in \R^{n \times n}$ such that 

\[\max\{\|C - \hat{C} T\|_F, \| B - T^{-1} \hat{B}\|_F\} \leq 5\sqrt{n \| G - \hat{G}\|}
\]
 and 
 \[\|A - T^{-1} \hat{A}T\|_F \leq \frac{\sqrt{n \|G - \hat{G}\|} \| H\| }{\sigma_{min}^{3/2}(H^{-})}\]
 
 and 
 \[\Norm{D - \hat{D}}_F \leq \sqrt{n}\Norm{G - \hat{G}}\]
 where in the above
 \[
 G = [D, CB, CAB, ..., CA^{2s-1}B]  \,.
 \]
\end{theorem}


Putting together the above theorems, we can prove our main result.

\begin{proof}[Proof of Theorem~\ref{thm:main-thm}]
The proof follows from simply combining the theorems above (rescaling $\eps$ appropriately by a polynomail in the other parameters) and observing that the running time is a fixed polynomial in the number of samples $N$, once $$N \geq \poly\Paren{ m, n, p, s, \kappa, 1/w_{\min} , 1/\eps, 1/\gamma , 1/\delta }.$$ 

\end{proof}


Next, we focus on proving each intermediate theorem. 

\textcolor{red}{Need to rewrite proofs from here and below but should be straight-forward.  Section~\ref{sec:jennrichalg} has the guarantees for Jennrich's algorithm that we can use black-box.  The proofs I had in mind are as follows
\begin{enumerate}
\item For Theorem~\ref{thm:span-recovery}, we prove linear independence of the factors using joint nondegeneracy then invoke Jennrich's algorithm
\item For Theorem~\ref{thm:block-henkel-recovery} we again use linear independence to argue that the right set of weights is essentially ``unique"
\item With these two theorems filling out the rest should be trivial
\end{enumerate}
}


\subsection{Proof of Theorem \ref{thm:span-recovery} }


We first show that the empirical  $6$-th moment tensor is close to the true tensor in Frobenius norm.

\begin{lemma}[Empirical Concentration of the 6-th Moment]\label{lem:empirical-estimate-tensor}
Given $\eps, \delta>0$ and $N\geq N_0$ length $6s$ trajectories from a mixture of linear dynamical systems $\calM = \sum_{i\in [k]} w_i \calL(A_i, B_i, C_i, D_i)$, if 
\[
N_0 \geq \poly(m,n,p,s ,  \kappa, 1/w_{\min}, 1/\gamma, 1/\eps, 1/\delta ),
\]
with probability at least $1-\delta$
Algorithm~\ref{algo:learning-subspaces} outputs a tensor $\wh{\Pi}_{\calM}$ such that
\[
\Norm{\wh{\Pi}_{\calM}  - \Pi_{\calM}}_F \leq \eps ,
\]
where $\Pi_{\calM} = \sum_{i \in [k]}  w_i G_{\calL_i, 2s} \otimes G_{\calL_i, 2s} \otimes G_{\calL_i, 2s}$.
\end{lemma}
\begin{proof}
Note that the joint distribution of $(u_1^i, \dots , u_l^i, y_1^i , \dots , y_l^i)$ is Gaussian.  Furthermore, the covariance of this Gaussian has entries bounded by $\poly(m,n,p,s,\kappa)$.  Thus, by standard concentration inequalities, the empirical sixth moment tensor concentrates around its mean with high probability.  Since $\Pi_{\calM}, \wh{\Pi}_{\calM}$ are obtained by taking a linear transformation of the sixth moment tensor and the coefficients of this transformation are also bounded by $\poly(m,n,p,s,\kappa)$, we are done.



\ainesh{the proof isn't that straight-forward here...we need to compute the variance of the estimator $\hat{T}_{k_1,k_2,k_3}$ from Algorithm 5.1 and show it is bounded. }
\end{proof}

Next, we show that running Jennrich's algorithm on an appropriate flattening of the tensor $\wh{P}_{\calM}$ recovers an estimate of the Markov parameters of each individual component of the mixture.

\begin{lemma}[Markov Parameters via Tensor Decomposition]\label{lem:decompose-tensor}
Given $\eps, \delta>0$ and $N\geq N_0$ length $6s$ trajectories from a mixture of linear dynamical systems $\calM = \sum_{i\in [k]} w_i \calL(A_i, B_i, C_i, D_i)$, if 
\[
N_0 \geq \poly(m,n,p,s ,  \kappa, 1/w_{\min}, 1/\gamma, 1/\eps, 1/\delta ),
\]
with probability at least $1-\delta$, Jennrich's algorithm (Algorithm~\ref{algo:jennrich}) outputs tensors $\wh{T}_1, \wh{T}_2, \ldots , \wh{T}_k$ such that there is some permutation $\pi$ on $[k]$ such that for all $i \in [k]$,
\[
\Norm{\wh{T}_{\pi(i)} - w_i \cdot  v(G_{\calL_i, 2s}) \otimes v(G_{\calL_i, 2s}) \otimes v(G_{\calL_i, 2s})}_F \leq \eps, 
\]
where  $v(G_{\calL_i, 2s})$ denotes flattening the matrix $G_{\calL_i, 2s}$ into a $mp(2s+1)$-dimensional vector.
\end{lemma}
\begin{proof}
Let $K$ be the matrix whose columns are $v(G_{\calL_i, 2s})$.  By the joint nondegeneracy assumption, $\sigma_k(K) \geq \gamma$ \ainesh{wait why is this the case? somehow for $k=2$, this is going from a square matrix to a matrix with $2$ columns, and the singular value is lower bounded?}.  On the other hand, we know that 
\[
\norm{K}_F \leq \poly(k,m,p,n,s, \kappa)
\]
so we can apply Theorem~\ref{thm:robust-jennrich} and Lemma~\ref{lem:empirical-estimate-tensor} (with $\eps$ rescaled appropriately by a polynomial in the other parameters) to get the desired bound.
\end{proof}




Now we can complete the proof of Theorem~\ref{thm:span-recovery}.
\begin{proof}[Proof of Theorem~\ref{thm:span-recovery}]
Lemma~\ref{lem:decompose-tensor} implies that  
\[
\norm{\wh{v}_i - w_i \cdot v(G_{\calL_i, 2s}) \norm{v(G_{\calL_i, 2s} }^2 } \leq \eps \,.
\]
This also implies that 
\[
\left \lvert \norm{\wh{v}_i} - w_i \norm{v(G_{\calL_i, 2s} }^3 \right \rvert \leq \eps \,.
\]
Also note that we must have
\[
1 \leq \norm{v(G_{\calL_i, 2s})} \leq \poly(k,m,n,p,s, \kappa) \,.
\]
Thus
\[
\norm{\wh{v}_i/\norm{\wh{v}_i}^{2/3} - w_i^{1/3} v(G_{\calL_i, 2s})  } \leq \eps \cdot \poly(k,m,n,p,s, \kappa) \,.
\]
We now get the desired bound by simply rescaling the setting of $\eps$ in Lemma~\ref{lem:decompose-tensor} by a polynomial in the other parameters.
\end{proof}



\subsection{Proof of Theorem~\ref{thm:block-henkel-recovery}}


\begin{proof}[Proof of Theorem~\ref{thm:block-henkel-recovery}]
Recall by Fact~\ref{fact:markov-params-formula} and Definition~\ref{def:estimator-means} that $\EE[\wh{R}_{\calM}] = R_{\calM}$.  Also by the same argument as in the proof of Lemma~\ref{lem:empirical-estimate-tensor}, the empirical estimate concentrates with high probability since the observations and control inputs are jointly Gaussian with bounded covariance.  Thus, with $1 - \delta$ probability, we have $\norm{ R_{\calM} - \wh{R}_{\calM}}_F \leq \eps$.  Recalling the definition of $R_{\calM}$ and applying Theorem~\ref{thm:span-recovery}, we must have that
\[
\norm{ \wh{R}_{\calM} - w_i^{2/3}\wt{G}_{\pi(i)}}_F \leq \eps (k + 1) \,.  
\]
Now consider any other set of choices for $\wt{w}_{\pi(i)}$.  We must have that 
\[
\norm{ \sum_{i = 1}^k(w_i^{2/3} - \wt{w}_{\pi(i)})\wt{G}_{\pi(i)}}_F \leq 2(k + 1)\eps \,.
\]
On the other hand we can write
\[
\norm{\sum_{i = 1}^k (w_i^{2/3} - \wt{w}_{\pi(i)})\wt{G}_{\pi(i)}}_F \geq \norm{\sum_{i = 1}^k(w_i^{2/3} - \wt{w}_{\pi(i)}) w_i^{1/3}G_{\calL_i, 2s}}_F - \eps \sum_{i = 1}^k |w_i^{2/3} - \wt{w}_{\pi(i)}| \,.
\]
Now for any coefficients $c_1, \dots , c_k$, we have
\[
\begin{split}
\norm{c_1G_{\calL_1, 2s} + \dots + c_k G_{\calL_k, 2s}}_F \geq  \frac{\gamma(|c_1| + \dots + |c_k|)}{\sqrt{k}}  
\end{split}
\]
where we used the joint nondegeneracy assumption.  Thus,
\[
\begin{split}
\norm{\sum_{i = 1}^k (w_i^{2/3} - \wt{w}_{\pi(i)})\wt{G}_{\pi(i)}}_F  \geq \frac{\gamma w_{\min}^{1/3} \sum_{i = 1}^k |w_i^{2/3} - \wt{w}_{\pi(i)}|}{\sqrt{k}} - \eps \sum_{i = 1}^k |w_i^{2/3} - \wt{w}_{\pi(i)}| \\ \geq  \left(\frac{\gamma w_{\min}^{1/3}}{\sqrt{k}} - \eps \right) \max_{i} (|w_i^{2/3} - \wt{w_{\pi(i)}}| )\,. 
\end{split}
\]
Combining this with the previous inequality gives the desired bound.
\end{proof}







\subsection{Jennrich's Algorithm}\label{sec:jennrichalg}

Jennrich's Algorithm is an algorithm for decomposing a tensor, say $T= \sum_{i=1}^r (x_i \otimes y_i \otimes z_i)$, into its rank-$1$ components that works when the fibers of the rank $1$ components i.e. $x_1, \dots , x_r$ are linearly independent (and similar for $y_1, \dots , y_r$ and $z_1, \dots , z_r$).


Moitra \cite{moitra2018algorithmic} gives a complete analysis of {\sc Jennrich's Algorithm}.  The result that we need is that as the error $E$ goes to $0$ at an inverse-polynomial rate, {\sc Jennrich's Algorithm} recovers the individual rank-$1$ components to within any desired inverse-polynomial accuracy.  
\begin{theorem}[\cite{moitra2018algorithmic}]\label{thm:robust-jennrich}
Let 
\[
T = \sum_{i=1}^r \sigma_i (x_i \otimes y_i \otimes z_i)
\]
where the $x_i,y_i,z_i$ are unit vectors and $\sigma_1 \geq \dots \geq \sigma_r > 0$.  Assume that the smallest singular value of the matrix with columns given by $x_1, \dots, x_r$ is at least $c$ and similar for the $y_i$ and $z_i$.  Then for any constant $d$, there exists a polynomial $P$ such that if
\[
\norm{E}_2 \leq  \frac{\sigma_1}{P(n, \frac{1}{c}, \frac{\sigma_1}{\sigma_r})}
\]
then with $1 - \frac{1}{(10n)^d}$ probability, there is a permutation $\pi$ such that the outputs of {\sc Jennrich's Algorithm} satisfy
\[
\norm{\sigma_{\pi(i)} (x_{\pi(i)} \otimes y_{\pi(i)} \otimes z_{\pi(i)}) - u_i \otimes v_i \otimes w_i}_2 \leq \sigma_1\left(\frac{\sigma_r c}{10\sigma_1 n}\right)^d
\]
for all $1 \leq i \leq r$.
\end{theorem}
\begin{remark}
Note that the extra factors of $\sigma_1$ in the theorem above are simply to deal with the scaling of the tensor $T$.  
\end{remark}


\subsection{Bayes Optimal Clustering}


In this section, we show that our parameter learning algorithm actually allows us to do nearly Bayes-optimal clustering in the fully observed case i.e. when $C_i = I$ for all $i \in [k]$ 
\begin{remark}
We believe our results naturally generalize to the partially observed setting as long as assume that all of the $\calL_i = \calL(A_i,B_i,C_i,D_i)$ are written in their balanced realization (see \cite{oymak2019non} for a formal definition) which is just a canonical choice of the similarity transformation $U_i$ that is allowed to act on $A_i,B_i,C_i$.
\end{remark}

\begin{theorem}\label{thm:optimal-clustering}
Let $\calM = w_1\calL_1 + \dots + w_k \calL_k$ be a mixture of LDS where each $\calL_i = \calL(A_i,B_i,C_i,D_i)$ with $C_i = I$ and assume that the mixture $\calM$ satisfies the assumptions in Section~\ref{sec:formal-setup}.  Then given 
\[
N = \poly\Paren{m,n,p , s, \kappa, 1/w_{\min} ,  1/\gamma,  1/\delta}
\]
sample trajectories from this mixture, there is an algorithm that runs in $\poly(N)$ time and has the following guarantees with probability $1 - \delta$.  There is a fixed permutation $\pi$ on $[k]$ such that given any trajectory $(u_1, \dots , u_l, y_1, \dots , y_l)$ with $l \leq O(s)$ and $\norm{u_i}, \norm{y_i} \leq \poly(m,n,p,s, \kappa, 1/w_{\min} ,  1/\gamma, 1/\delta)$ it computes a posterior distribution $(p_1 , \dots , p_k)$ on $[k]$ (with $p_1 + \dots + p_k = 1$) such that $(p_{\pi(1)}, \dots , p_{\pi(k)})$ is $\delta$-close in TV distance to the posterior distribution on $\calL_1, \dots , \calL_k$ from which the trajectory $(u_1, \dots , u_l, y_1, \dots , y_l)$ was drawn.  
\end{theorem}
\begin{remark}
Note that  $\norm{u_i}, \norm{y_i} \leq \poly(m,n,p,s, \kappa, 1/w_{\min} ,  1/\gamma, 1/\delta)$ is satisfied with exponentially small failure probability for a random trajectory from any of the components since $l \leq O(s)$.  The trajectories used in the learning algorithm have length $O(s)$ so in particular, we can nearly-optimally cluster those.
\end{remark}
\begin{proof}
We apply Theorem~\ref{thm:main-thm} with $\eps$ set as a sufficiently small inverse polynomial in the other parameters.  Because $C_i = I$, we can eliminate the similarity transformations $U_i$ and also WLOG the permutation $\pi$ on $[k]$ is the identity so we have
\[
\max_{i \in [k]}\left( \norm{A_i - \wh{A}_i }, \norm{B_i - \wh{B}_i }, \norm{C_i - \wh{C}_i }, \norm{D_i - \wh{D}_i }, |w_i - \wh{w}_i|  \right) \leq \eps \,.
\]
Now fix a choice of $i \in [k]$.  Define $\calP_i$ to be the probability that $(u_1, \dots u_l, y_1, \dots , y_l)$ is sampled from the LDS $\calL(A_i,B_i,C_i,D_i)$ and let $\wh{\calP}_i$ be the probability that it is sampled from the LDS $\wh{\calL}_i = \calL(\wh{A}_i, \wh{B}_i, \wh{C}_i, \wh{D}_i)$.  We can explicitly compute $\wh{\calP}_i$ from $\wh{A}_i, \wh{B}_i, \wh{C}_i, \wh{D}_i$ using regression.  Now we will bound the ratio $\calP_i/\wh{\calP}_i$ and prove that it is close to $1$.  We can write $\calP_i$ as an integral over all possibilities for $x_1, \dots , x_l$.  Now the likelihood of $(u_1, \dots u_l, y_1, \dots , y_l, x_1, \dots , x_l)$ is simply 
\[
C\exp\left( -\frac{1}{2}\left( \sum_{t= 1}^{l-1} \norm{x_{t+1} - A_ix_t - B_iu_t }^2 + \sum_{t = 1}^l \norm{y_t - C_ix_t  - D_iu_t}^2 + \sum_{t = 1}^l \norm{u_t}^2 \right) \right) 
\]
where $C$ is an appropriate normalizing constant obtained from the standard normal.  The formula is the same for $\wh{\calP}_i$ except with $A_i,B_i,C_i,D_i$ replaced with $\wh{A}_i, \wh{B}_i, \wh{C}_i, \wh{D}_i$.  As long as 
\[
\norm{x_1}, \dots , \norm{x_l} \leq \poly(m,n,p,s, \kappa, 1/w_{\min} ,  1/\gamma, 1/\delta)
\]
then the ratio between the two likelihoods is in the interval $[1 - \sqrt{\eps}, 1 + \sqrt{\eps}]$ as long as $\eps$ was chosen sufficiently small initially.  However, the above happens with exponentially small failure probability for both $\calL_i$ and $\wh{\calL}_i$ so we actually have
\[
1 - 2\sqrt{\eps} \leq \frac{\wh{\calP}_i}{\calP_i} \leq 1 + 2\sqrt{\eps} \,.
\]
Combining the above over all $i \in [k]$ immediately implies the desired statement about the posterior distribution.
\end{proof}


==> new-setup.tex <==
\section{Technical Overview}
A linear dynamical system $\calL$ is defined as follows.  A state vector $x_t$ indexed by timesteps $t \in [l]$ transitions according to the following markov process.  
\begin{equation*}
\begin{split}
    x_{t+1} &= A x_{t} + B u_t + w_t ,\\
    y_{t} &= C x_t + D u_t + z_t ,
\end{split}
\end{equation*}
Here $A,B,C,D$ are matrices with dimensions  $n \times n$, $n \times p$, $m \times n$ and $m \times p$ respectively.  The random variables $w_t$ and $z_t$ are typically modeled as standard normal corresponding to process and measurement noise.  In the most general setting, $\{y_t\}_{t \in [l]}$ is the dataset from which we wish to infer the system parameters $A,B,C,$ and $D$.  Note that it is only possible to recover the system parameters under an equivalence class of similarity transforms.  A standard recipe for this task is the algorithm of Ho-Kalman which succeeds at recovering $\hat{A}$ such that there exists a similarity transform $U$ satisfying $\Norm{A - U\hat{A}U^{-1}} = 0$ with analogous guarantees for $\hat{B}, \hat{C},$ and $\hat{D}$ in infinite samples.  The crux of the Ho-Kalman algorithm is to first estimate "markov parameters" of the form $CA^iB$ for varying values of $i \in \Z^+$.  The markov parameters are arranged in a corresponding Hankel matrix and an SVD style procedure is applied to the Hankel matrix to recover the system parameters.  The key is to estimate markov parameters which is difficult when the data $\{y_t\}_{t \in [l]}$ is drawn from a mixture of linear dynamical systems defined next.  

\begin{definition}[Mixture of Linear Dynamical System]
\label{definition:mixture-of-LDS}
 A mixture of linear dynamical systems is represented as $\calM = w_1 \calL_1 + \dots w_k \calL_k$, where $w_1 , \dots , w_k$ are positive real numbers summing to $1$ and $\calL_1((A_1,B_1,C_1,D_1), \dots , \calL_k(A_k, B_k,C_k,D_k)$ are each individual linear dynamical systems with the same dimensions (i.e. the same $m,n,p$).  The trajectories we observe are sampled according to the following process.  First an index $i \in [k]$ is drawn according to the mixing weights $w_1, \dots , w_k$ and then a trajectory of length $s$, denoted by $\{ y_1, \dots , y_s \}$ is drawn from the corresponding dynamical system $\calL_i$. 
\end{definition}
Our goal is to learn the parameters of the mixture, i.e.    
the individual linear dynamical systems and their mixing weights, given polynomially many samples from the mixture.  In this setting, if the trajectory length $s$ is large enough for the system parameters to be learned from a single trajectory then it would be possible to learn each dynamical system $\calL$ separately which trivializes the problem.  The question is whether we can learn the markov parameters when $s$ is small. Our general strategy is as follows.  For a particular markov parameter $CA^{i}B$ we compute the order 6-tensor $ y_{t+3i+2}\otimes u_{t+2i+2} \otimes y_{t + 2i + 1} \otimes u_{t + i + 1} \otimes  y_{t + i} \otimes u_{t} $, and aggregating over all trajectories we obtain an estimate of the following four tensor denoted $T_{i}$     
\[T_{i} \defeq
\EE\left[ y_{t+3i+2}\otimes u_{t+2i+2} \otimes y_{t + 2i + 1} \otimes u_{t + i + 1} \otimes  y_{t + i} \otimes u_{t} \right] = \sum_{j \in [k]}w_jC_jA_j^{i}B_j \otimes  C_jA_j^{i}B_j \otimes  C_jA_j^{i}B_j
\,.
\]
Brushing aside issues of sample complexity,
given the above 6-tensor $T_{i}$ exactly then we can flatten the tensor along its first and second, third and fourth, and fifth and sixth modes to obtain a three tensor.  Although this step is largely cosmetic, it then enables us to apply Jenrich's algorithm for decomposing three tensors to recover the markov parameter $C_jA_j^iB_j$.  Applying this approach to varying values of $i$ recovers the full set of markov parameters and enables the success of Ho-Kalman for learning the system parameters $A,B,C,D$. 




\section{Formal Setup}
\label{sec:formal-setup}

A linear dynamical system $\calL$ is defined as follows. At each time step $t$ there is an unknown hidden state $x_t \in \mathbb{R}^n$ and a known exogenous input $u_t \in \mathbb{R}^p$. The transition dynamics and observations $y_t \in \mathbb{R}^m$ are generated according to the following rules:
\begin{equation*}
\begin{split}
    x_{t+1} &= A x_{t} + B u_t + w_t ,\\
    y_{t} &= C x_t + D u_t + z_t ,
\end{split}
\end{equation*}
Here $A$, $B$, $C$ and $D$ are matrices of dimension $n \times n$, $n \times p$, $m \times n$ and $m \times p$ respectively. Moreover $w_t$ and $z_t$ are independent random variables and are called the process and observation noise respectively. It is standard to assume that they, along with the inputs and the initial state $x_0$, are all Gaussian, though we will work in a more general setting.



\begin{model}[Linear Dynamical System]
\label{model:LDS}
 Let $A \in \mathbb{C}^{n \times n}$, $B \in \mathbb{C}^{n \times p}$,  $C \in \mathbb{C}^{m \times n}$, and $D\in \mathbb{C}^{m \times p}$ be complex valued matrices. Let $\calD_0$, $\calD_{u}$, $\calD_{w}$, $\calD_{z}$ be distributions with mean zero. Then, a Linear Dynamical System, $\calL\Paren{A,B,C,D}$, is defined as follows: 
\begin{equation*}
\begin{split}
    x_{t+1} &= A x_{t} + B u_t + w_t ,\\
    y_{t} &= C x_t + D u_t + z_t ,
\end{split}
\end{equation*}
where $x_0 \sim \calD_{0}$, and for all $t\in\mathbb{N}$,  $u_t \sim \calD_{u} $, $w_t \sim \calD_{w}$ and $z_t \sim \calD_{z}$. 
\end{model}


For simplicity, throughout this paper, we will consider when all of the noise distributions are isotropic Gaussians i.e. $\calD_0 = N(0, I_n), \calD_u = N(0, I_p) , \calD_w = N(0, I_n), \calD_z = N(0, I_m)$ although our results generalize to more general noise distributions as long as they have sufficiently many bounded moments.  



\paragraph{Mixtures of Linear Dynamical Systems.}
We extend the above model to a setting where the input observations are generated from a mixture of linear dynamical systems. Formally,



\begin{model}[Mixture of Linear Dynamical System]
\label{model:mixture-of-LDS}
 A mixture of linear dynamical systems is represented as $\calM = w_1 \calL_1 + \dots w_k \calL_k$, where $w_1 , \dots , w_k$ are positive real numbers summing to $1$ and $\calL_1((A_1,B_1,C_1,D_1), \dots , \calL_k(A_k, B_k,C_k,D_k)$ are each individual linear dynamical systems with the same dimensions (i.e. the same $m,n,p$).  The trajectories we observe are sampled according to the following process.  First an index $i \in [k]$ is drawn according to the mixing weights $w_1, \dots , w_k$ and then a trajectory of length $s$, denoted by $\{ y_1, \dots , y_s \}$ is drawn from the corresponding dynamical system $\calL_i$. 
\end{model}

Our goal is to learn the parameters of the mixture, i.e. the individual linear dynamical systems and their mixing weights, given polynomially many samples from the mixture.

\subsection{Assumptions for Learnability}
\label{subsec:assumptions}
We begin with standard definitions of the observability and controllability matrix of a single LDS.  The condition number of these matrices governs the non-degeneracy of a single LDS.  In particular, we need to assume that they are non-degenerate for even learning a single LDS to be possible.  

\begin{definition}[Observability Matrix]\label{def:observability}
For an LDS $\calL(A,B,C,D)$ and an integer $s$, define the matrix $O_{\calL, s} \in \R^{sm \times n}$ as
\begin{equation*}
    O_{\calL, s} =\begin{bmatrix} C  \\  CA \\ \ldots \\ CA^{s-1} \end{bmatrix}.
\end{equation*}
\end{definition}
A LDS is \emph{observable} if for some $s$, the matrix $O_s$ has full column-rank. 
Similarly, we need to ensure that the control input is not degenerate, and only acts in a subspace that is not spanned by $A$. This is made precise by considering the \emph{controllability matrix}: 
\begin{definition}[Controllability Matrix]\label{def:controllability}
For an LDS $\calL(A,B,C,D)$ and  an integer $s$, define the matrix $Q_{\calL, s} \in \R^{n \times sp}$ as
\begin{equation*}
    Q_{\calL, s} = \begin{bmatrix} B & AB & \ldots & A^{s-1} B\end{bmatrix}
\end{equation*}
\end{definition}
A LDS is \emph{controllable} if the controllability matrix has full row-rank. These two assumptions are necessary for the LDS to be learnable and in fact it is necessary to make a quantitatively robust assumption of this form (see \cite{bakshi2023new}).  In other words, we need a bound on the condition number of the observability and controllability matrices.

In addition to the assumptions required to learn a single linear dynamical system, we will require addition assumptions on the interaction of the LDS's to obtain learning algorithms for the mixture (as otherwise there could be degeneracies such as two components being almost the same which would make it information-theoretically impossible to learn).  

\subsubsection{Joint Nondegeneracy}

We introduce a  joint nondegeneracy condition that prevents certain degeneracies arising from the interaction between the components of the mixture e.g. if the components are too close to each other. 

\begin{definition}[Markov Parameters]
\label{def:markov-params}
Given a linear dynamical system, $\calL\Paren{ A,B, C,D}$, and an integer $T\geq 1$, the Markov Parameter matrix $G_{\calL, T}\in \R^{m \times (T + 1)p} $ is defined as the following block matrix:
\begin{equation*}
    G_{\calL, T} = \begin{bmatrix}
    D &  CB &  CAB &  \ldots & CA^{T-1}B
    \end{bmatrix}. 
\end{equation*}
\end{definition}


\begin{definition}[Joint Nondegeneracy]\label{thm:jointnd}
For a mixture of LDS $\calM = w_1 \calL_1 + \dots + w_k \calL_k$ where each individual LDS is given by $\calL_i = \calL(A_i, B_i,C_i,D_i)$ (with the same dimension parameters $m,n,p$), we say $\calM$ is $(\gamma,s)$-jointly nondegenerate if for any real numbers $c_1, \dots , c_k$ with $ c_1^2 + \dots + c_k^2 = 1$, we have
\[
\norm{ c_1 G_{\calL_1, s} + \dots + c_k G_{\calL_k, s}} \geq \gamma \,.
\]
\end{definition}







We make the following assumptions about the mixture $\calM$ that we are trying to learn.

\begin{definition}[Well Behaved Mixture of LDS]\label{def:well-behaved-mixture}
We say a mixture of LDS $\calM = w_1 \calL_1 + \dots + w_k \calL_k$ where each $\calL_i = \calL(A_i,B_i,C_i,D_i)$ is well-behaved if the following assumptions hold
\begin{itemize}
\item \textbf{Non-trivial Mixing Weights:} for some $w_{\min} > 0$, we have $w_i \geq w_{\min}$ for all $i \in [k]$

\item \textbf{Non-trivial Individual Controllers and Measurements:} for all $i \in [k]$, $\norm{B_i}, \norm{C_i} \geq 1$
\item \textbf{Individual Boundedness:} for some parameter $\kappa$,
\[
\norm{A_i}, \norm{B_i}, \norm{C_i}, \norm{D_i} \leq \kappa \text{ for all } i \in [k]
\]
\item \textbf{Individual Observability and Controllability:}  for some integer $s$ and parameter $\kappa$, for all $i \in [k]$ the matrix $O_{\calL_i,s}$ has full column rank, the matrix $Q_{\calL_i, s}$ has full row rank and
 \begin{equation*}
        \begin{split}
            \sigma_{\max}(O_{2s})/\sigma_{\min}(O_s) &\leq \kappa, \\
            \sigma_{\max}(Q_{2s})/\sigma_{\min}(Q_s) &\leq \kappa.
        \end{split}
\end{equation*}
\item \textbf{Joint Nondegeneracy:} The mixture $\calM$ is $(\gamma,s)$ jointly nondegenerate
\end{itemize}
\end{definition}

The assumptions on the individual components mirror those in \cite{bakshi2023new} where a more detailed discussion and justification can be found.  We have the following two claims from \cite{bakshi2023new} that give us bounds on the singular values of $O_{\calL_i, s}, Q_{\calL_i,s}, A^s$. 
\begin{claim} \cite{bakshi2023new}\label{claim:eigenvalue-bound}
Consider a well-behaved mixture of LDS (Definition~\ref{def:well-behaved-mixture}) $\calM = w_1 \calL_1 + \dots + w_k \calL_k$ where each $\calL_i = \calL(A_i,B_i,C_i,D_i)$. Then for all $i$, $\sigma_{\min}(O_{\calL_i,s}) \leq \sqrt{s}\kappa$ and  $\sigma_{\min}(Q_{\calL_i,s}) \leq \sqrt{s}\kappa$.
\end{claim}

\begin{claim}\cite{bakshi2023new}\label{claim:boundA} Consider a well-behaved mixture of LDS (Definition~\ref{def:well-behaved-mixture}) $\calM = w_1 \calL_1 + \dots + w_k \calL_k$ where each $\calL_i = \calL(A_i,B_i,C_i,D_i)$.  Then for any integer $t > 0$,
\[
\norm{A_i^t}_F \leq (\sqrt{n} \kappa)^{t/s} \,. 
\]
\end{claim}















\section{Basic Properties}

We begin with some basic properties of a single linear dynamical systems $\calL = \calL(A,B,C,D)$.  






%\begin{definition}[Canonical Block Henkel Matrix]
%\label{def:canonical-block-henkel}
%Given the Markov parameters of linear dynamical system $\calL(A,B,C,D)$, let $H_{\calL}$ be a block Henkel matrix corresponding to $\calL$ defined as follows:
%\begin{equation*}
%H_{\calL}= \begin{bmatrix} D & CB & \ldots & CA^{k-2} B\\
%CB & CAB & \ldots & CA^{k-1}B\\
%\vdots& \vdots& \vdots &\vdots \\
%CA^{k-2}B & CA^{k-1}B & \ldots & CA^{2k-3} B.
%\end{bmatrix}
%\end{equation*}
%\end{definition}




\begin{fact}[Algebraic Identities for LDS's]\label{fact:formula}
Let  $\calL\Paren{A,B,C,D }$ be a Linear Dynamical System. Then, for any $t \in \mathbb{N}$, 
\begin{equation*}
    y_t = \sum_{i = 1}^{t} \Paren{  C A^{i-1} B   u_{t-i}  + C A^{i-1}w_{t-i} } + CA^{t}x_0 +  Du_t + z_{t} \,.
\end{equation*}
\end{fact}


\begin{fact}[Cross-Covariance of Control and Observation]\label{fact:markov-params-formula}
For any $t,k \in \mathbb{N}$, and any $0 \leq j \leq k$, given observations $y_t$ and control inputs $u_t$ from a linear dynamical system $\calL(A,B,C,D)$ such that $\expecf{}{u_t u_t^\top} =I$ and the $u_t$'s are independent, we have  
    \begin{equation*}
        \expecf{}{y_{t+j} u_t^\top } =  \begin{cases} D \text{ if } $j = 0$ \\
        C A^{ j - 1} B \text{ otherwise}
        \end{cases}
    \end{equation*}
\end{fact}
\begin{proof}
Invoking the algebraic identity from Fact~\ref{fact:formula}, consider the case where $j \neq 0$.
\begin{equation}
\label{eqn:expansion-2nd-moment}
\begin{split}
    \expecf{}{ y_{t+j} u_t^\top  } & = \expecf{}{  \Paren { \sum_{i = 1}^{t+j } \Paren{  C A^{i-1} B   u_{t+j-i}  + C A^{i-1}w_{t+j-i} } + CA^{t+j}x_0 +  Du_{t+j} + z_{t+j}  } u_t^\top } \\
    & = \underbrace{ \sum_{i = 1}^{j-1} CA^{i-1} B \expecf{}{u_{t+j-i} u_t^\top}   }_{\eqref{eqn:expansion-2nd-moment}.(1)}  + CA^{j-1} B \expecf{}{u_t u_t^\top }  + \underbrace{ \sum_{i = j+1}^{t+j} CA^{i-1} B \expecf{}{u_{t+j-i} u_t^\top} }_{\eqref{eqn:expansion-2nd-moment}.(2)}  \\
    & \hspace{0.2in} + \underbrace{ \sum_{i = 1}^{t+j } CA^{i-1} \expecf{}{w_{t+j-i} u_t^\top} + CA^{t+j} \expecf{}{ x_0 u_t^\top}  + D \expecf{}{ u_{t+j} u_t^\top } + \expecf{}{ z_{t+j }  u_t^\top} }_{ \eqref{eqn:expansion-2nd-moment}.(3) } \\
    & = CA^{j-1} B
\end{split}
\end{equation}
where the last inequality follows from observing that by independence of $u_t$'s,  $w_t$'s , $z_t$'s and $x_0$, the terms \eqref{eqn:expansion-2nd-moment}.(1), \eqref{eqn:expansion-2nd-moment}.(2) and \eqref{eqn:expansion-2nd-moment}.(3) are $0$. Similarly, when $j=0$, the only non-zero term is $\expecf{}{ D u_t u_t^\top } = D$ and the claim follows.
\end{proof}


In light of the above, we make the following definition. 
\begin{definition}[System Parameters]\label{def:estimator-means}
 For an LDS $\calL(A,B,C,D)$ and an integer $j \geq 0$, we define the matrix $X_{\calL, j}$ as 
\[
X_{\calL, j} =   \begin{cases} D \text{ if } $j = 0$ \\
C A^{ j - 1} B \text{ otherwise}
\end{cases} \,.
\]
\end{definition}
 It is easy to see that  $\EE[y_{t + j} u_t^\top ] = X_{\calL, j}$ by the previous fact.



\begin{lemma}[Sixth-moment Statistics]\label{lem:fourthmoment}
Given a linear dynamical system $\calL(A, B , C, D)$ and integers $t, k_1, k_2, k_3 \geq 0$, we have
\begin{equation*}
\expecf{}{y_{t + k_1 + k_2 + k_3 + 2} \otimes u_{t + k_1 + k_2 + 2} \otimes y_{t + k_1 + k_2 + 1} \otimes u_{t + k_1 + 1} \otimes  y_{t + k_1} \otimes u_{t}  } = X_{\calL, k_3} \otimes X_{\calL, k_2} \otimes  X_{\calL, k_1} \,, 
\end{equation*}
where $X_{\calL,j}$ is defined in Definition~\ref{def:estimator-means}. 
\end{lemma}
\begin{proof}
First, for simplicity consider the case where $k_1=  k_2 = k_3 =0$. Then, 

\begin{equation}
\begin{split}
    \expecf{}{ y_{t + 2}  \otimes u_{t+ 2} \otimes y_{t+ 1} \otimes u_{t+1} \otimes y_{t} \otimes u_t } &  = \expecf{}{ D u_{t+2} \otimes u_{t+2} \otimes D u_{t+1} \otimes u_{t+1} \otimes D u_t \otimes u_t } \\
    & = \Paren{ D \expecf{}{u_{t+2 } u_{t+2}^\top } }  \otimes \Paren{ D \expecf{}{u_{t+1 } u_{t+1}^\top } }  \otimes \Paren{ D \expecf{}{u_{t } u_{t}^\top } } \\
    & = D \otimes D \otimes D,
\end{split}
\end{equation}
where the second equality follows from $u_{t+2}, u_{t+1}$ and $u_{t}$ being independent random variables. 
Next, consider the case where $k_3=0$ and $k_2, k_1 >0$. Observe, $y_{t+k_1 + k_2 + 2} \otimes u_{t+ k_1 + k_2 + 2}$ has only one non-zero term in expectation. Therefore, we can split the sum as follows: 

\begin{equation}
\label{eqn:k-3=0}
    \begin{split}
    & \expecf{}{ y_{t+ k_1 + k_2 +2  } \otimes u_{t+k_1 +k_2 + 2}  \otimes y_{t+k_1 + k_2 + 1} \otimes u_{t+k_1 + 1}  \otimes y_{t+k_1} \otimes u_{t}  } \\
    & = \expecf{}{ D \Paren{ u_{t+ k_1 + k_2 + 2 }\otimes u_{t+ k_1 + k_2 + 2 } }  \otimes \Paren{ y_{t+k_1 + k_2 + 1}  \otimes  u_{t+k_1 + 1}   } \otimes \Paren{y_{t+k_1} \otimes u_{t }}  }  \\
    & = D \Paren{ \expecf{}{u_{t+ k_1 + k_2 + 2 }\otimes u_{t+ k_1 + k_2 + 2 }}  } \otimes \underbrace{ \expecf{}{ \Paren{ y_{t+k_1 + k_2 + 1}  \otimes  u_{t+k_1 + 1}    } \otimes \Paren{y_{t+k_1} \otimes u_{t}}  } }_{\eqref{eqn:k-3=0}.(1) }  \\
    \end{split}
\end{equation}
where the second equality follows from observing that $u_{t+k_1 +k_2 + 2}$ is independent of all the terms appearing in the expansion of $y_{t+k_1+k_2 +1}$  and $y_{t+k_1}$, and the random variables $u_{t+ k_1 + k_2 + 2}$ and $u_{t+k_1}$. 

Now, we focus on simplifying term \eqref{eqn:k-3=0}.(1). Let $\zeta_t = CA^t x_0 + Du_t + z_t$. Observe that $\expecf{}{ w_t \otimes u_{t'} } = \expecf{}{ CA^t x_0 \otimes u_t }= \expecf{}{ z_t \otimes u_t }  = 0$,  for all $t,t'$, and $\expecf{}{ u_{t_1} \otimes u_{t_2} \otimes u_{t_3} \otimes u_{t_4}  } = 0$ for all $t_1> t_2 > t_3 > t_4$. Further, any permutation of $t_1, t_2, t_3$ and $t_4$ is also $0$.  Plugging in the definition from Fact \ref{fact:formula},  we have
\begin{equation}
\label{eqn:4-th-tensor}
    \begin{split}
        & \EE \Big[  y_{t+k_1 + k_2 + 1} \otimes u_{t + k_1 + 1} \otimes y_{t + k_1} \otimes u_t \Big]  \\
        & = \EE \Bigg[ \Paren{ \sum_{i = 1}^{t+k_1 +k_2 +1 } \Paren{  C A^{i-1} B   u_{t+k_1 +k_2 +1 -i}  + C A^{i-1}w_{t+k_1 +k_2 +1 -i} } + \zeta_{t+k_1 +k_2 +1 } } \otimes u_{t+k_1 + 1}  \\
        & \hspace{0.6 in} \otimes \Paren{\sum_{i = 1}^{t+k_1  } \Paren{  C A^{i-1} B   u_{t+k_1   -i}  + C A^{i-1}w_{t+k_1   -i} } + \zeta_{t+k_1   }   } \otimes  u_t \Bigg] \\
        &  = \EE \Bigg[ \Paren{ \sum_{i = k_2}^{t+k_1 +k_2 +1 } \Paren{  C A^{i-1} B   u_{t+k_1 +k_2 +1 -i}   }  } \otimes u_{t+k_1 + 1}  \\
        & \hspace{0.6  in} \otimes \Paren{\sum_{i = 1}^{t+k_1  } \Paren{  C A^{i-1} B   u_{t+k_1   -i}  + C A^{i-1}w_{t+k_1   -i} }    } \otimes  u_t \Bigg] \\
        & = \underbrace{ \EE \Bigg[ \Paren{  C A^{k_2-1} B       u_{t+k_1 +1 }  }  \otimes u_{t+k_1 + 1} \Bigg] }_{ \eqref{eqn:4-th-tensor}.(1) }  \otimes \underbrace{ \EE \Bigg[  \Paren{\sum_{i = 1}^{t+k_1  } \Paren{  C A^{i-1} B   u_{t+k_1   -i}  + C A^{i-1}w_{t+k_1   -i} }    } \otimes  u_t \Bigg]  }_{\eqref{eqn:4-th-tensor}.(2) } \\
        & \hspace{0.2 in}  + \underbrace{ \EE \Bigg[ \Paren{ \sum_{i = k_2+1}^{t+k_1 +k_2 +1 } \Paren{  C A^{i-1} B   u_{t+k_1 +k_2 +1 -i}   }  } \otimes u_{t+k_1 + 1}  \otimes    y_{t+k_1} \otimes  u_t \Bigg] }_{\eqref{eqn:4-th-tensor}.(3)}   
    \end{split}
\end{equation} 
where the second equality follows from observing that $\expecf{}{ w_{t+k_1 k_2 +1 -i } \otimes u_{t+ k_1 + 1} \otimes w_{t+ k_1 -j} \otimes u_t } = 0 $ for all $i \in [1, t+ k_1 + k_2 + 1 ]$ and $j \in [1, t+ k_1]$. Similarly, $\expecf{}{\zeta_{t+ k_1 + k_2 + 1} \otimes u_{t+k_1 + 1} \otimes  
y_{t+k_1}\otimes u_t } =0$. Further, for all $i \in [1, k_2 -1]$, $\expecf{}{ u_{t+k_1 + k_2 + 1 -i} \otimes u_{t+k_1 + 1} \otimes y_t \otimes u_t } =0$. The third equality follows from observing that $u_{t+k_1 + 1}$ is independent of $y_t \otimes u_t$.
Next, observe 
\begin{equation}
\label{eqn:4th.1}
    \eqref{eqn:4-th-tensor}.(1) =  CA^{k_2 - 1} B, 
\end{equation}
since $\expecf{}{u_{t+k_1 +1 } \otimes u_{t+k_1 +1 } } = I$. Using a similar argument, we observe that all the terms in \eqref{eqn:4-th-tensor}.(2) are zero in expectation apart from the one corresponding to $CA^{k_1-1}B$. Therefore, 
\begin{equation}
\label{eqn:4th.2}
\eqref{eqn:4-th-tensor}.(2) = CA^{k_1 - 1} B.
\end{equation}
Next, recall that $\expecf{}{u_t}=0$ for all $t$, and since $u_{t+k_1 + 1}$ is independent of all $u_{t'}$ where $t'<  t+ k_1+1$, 
\begin{equation}
\label{eqn:4th.3}
    \begin{split}
        \eqref{eqn:4-th-tensor}.(3) & =  0.
    \end{split}
\end{equation}
Similarly, when $k_1=0$,  $\eqref{eqn:4-th-tensor}.(1)= D$ and when $k_2=0$, $\eqref{eqn:4-th-tensor}.(2)= D$. 

Therefore, combining equations \eqref{eqn:4th.1},\eqref{eqn:4th.2} and \eqref{eqn:4th.3}, and plugging them back into equation \eqref{eqn:k-3=0}, we have 
\begin{equation}
   \begin{split}
     \expecf{}{ y_{t+ k_1 + k_2 +2  } \otimes u_{t+k_1 +k_2 + 2}  \otimes y_{t+k_1 + k_2 + 1} \otimes u_{t+k_1 + 1}  \otimes y_{t+k_1} \otimes u_{t}  } 
    & = D   \otimes  X_{\calL , k_2} \otimes X_{\calL,k_1}  \\
    \end{split} 
\end{equation}

It remains to consider the case where $k_3 >0$. We can now simply repeat the above argument and observe that instead of picking up the term $D u_{t+k_1 + k_2 + k_3 + 2  }$ from the expansion of $y_{t+k_1 + k_2 +k_3 +2}$, we now pick up the term $CA^{k_3-1} B u_{t+k_1 + k_2 + k_3 + 2  }$. This concludes the proof.
\end{proof}







\subsection{Mixtures of LDS}


Now consider a mixture of LDS $\calM = w_1\calL_1 + \dots  + w_k\calL_k $ where $\calL_i = \calL(A_i, B_i, C_i, D_i)$.  Using Lemma~\ref{lem:fourthmoment}, we have an expression for the adjusted fourth moments of the mixture.



\begin{corollary}\label{coro:mixture-fourthmoment}
For a mixture of LDS $\calM = w_1\calL_1 + \dots  + w_k\calL_k $ and for $t, k_1, k_2 \geq 0$
\[
\begin{split}
\EE_{\calM}\left[ y_{t + k_1 + k_2 + k_3 + 2} \otimes u_{t + k_1 + k_2 + 2} \otimes y_{t + k_1 + k_2 + 1} \otimes u_{t + k_1 + 1} \otimes  y_{t + k_1} \otimes u_{t}  \right]  = \sum_{i = 1}^k w_i X_{\calL_i, k_3} \otimes X_{\calL_i, k_2} \otimes  X_{\calL_i, k_1}
\end{split}
\]
\end{corollary}
\begin{proof}
This follows directly from Lemma~\ref{lem:fourthmoment}. 
\end{proof}



